Towards Environmentally Equitable AI via Geographical Load Balancing

Fueled by the soaring popularity of large language and foundation models, the accelerated growth of artificial intelligence (AI) models' enormous environmental footprint has come under increased scrutiny. While many approaches have been proposed to make AI more energy-efficient and environmentally friendly, environmental inequity -- the fact that AI's environmental footprint can be disproportionately higher in certain regions than in others -- has emerged, raising social-ecological justice concerns. This paper takes a first step toward addressing AI's environmental inequity by balancing its regional negative environmental impact. Concretely, we focus on the carbon and water footprints of AI model inference and propose equity-aware geographical load balancing (GLB) to explicitly address AI's environmental impacts on the most disadvantaged regions. We run trace-based simulations by considering a set of 10 geographically-distributed data centers that serve inference requests for a large language AI model. The results demonstrate that existing GLB approaches may amplify environmental inequity while our proposed equity-aware GLB can significantly reduce the regional disparity in terms of carbon and water footprints.

==> tex/background.tex <==
%\newpage
\section{Background}
% \ifsectionVspace \rSection \fi

While the embodied water footprint (e.g., manufacturing  of servers and GPUs for training AI models) not directly related to AI model training or inference is part of the lifecycle
assessment of environmental footprint and 
can be of independent interest,
 we focus on the \emph{operational} water footprint
of AI models directly associated with training and inference.
Thus, in what follows, we introduce the basics of data center infrastructure
and then describe the way that data centers (and hence, the hosted AI models)
consume water.

\begin{wrapfigure}{r}{0.4\textwidth}
	\centering 
	\includegraphics[trim=0 11.2cm 17.6cm 0, clip, width=1\linewidth]{figures/power_infra.pdf}
	\caption{Data center power infrastructure. } \label{fig:PowerHierarchy}
\end{wrapfigure}
\textbf{Data center power infrastructure.}
While data center power infrastructures vary from one to another,
a common infrastructure design follows the hierarchical tree type. As illustrated in Figure~\ref{fig:PowerHierarchy}, grid/utility power enters the data center through an automatic transfer switch (ATS) which switches over the main power supply to the backup generator in case of grid power failures. The ATS feeds power to a centralized (or distributed in some systems) uninterrupted power supply (UPS), which supplies ``protected/conditioned'' power to multiple power distribution units (PDUs) that further  deliver power to the computer servers.
 Meanwhile, the cooling system ensures that the servers are not overheated. 
The computer servers are where AI models are trained and deployed for inference. These servers may also have specialized designs, including
multiple GPUs and/or purpose-built hardware, to speed
up AI model training and inference \cite{ML_WorkloadAnalysis_MultiTenantGPU_Microsoft_ATC_2019_10.5555/3358807.3358888}.




\textbf{Data center water footprint.}
We first would like to distinguish water \emph{consumption} from \emph{withdrawal}. Water withdrawal refers to getting water from the source (e.g., underground, rivers, sea) \cite{macknick2011review}, and water consumption refers to ``losing'' water (e.g., by evaporation) in the process of withdrawal and return. Thus,
water consumption is the \emph{net} difference between water withdrawal and return. In this paper, we focus on water consumption, which is consistent with the industry standard \cite{GreenGrid_Whitepaper_WUE}. 
 The water consumption in data centers has two parts: \emph{on-site direct} water and \emph{off-site indirect} water.

\begin{wrapfigure}[16]{r}{0.5\textwidth}
	\vspace{-0.3cm}
	\centering 
    \includegraphics[trim=0 4.3cm 3.8cm 0, clip, width=1\linewidth]{figures/datacenter_water.pdf}
\caption{Data center water footprint: on-site water consumption
for data center cooling, and off-site water consumption
for electricity generation. Multiple AI models are trained and/or deployed in
the data center. The icons for AI models are only for illustration purposes.} \label{fig:water_footprint}
	\vspace{-0.3cm}
\end{wrapfigure}
\underline{On-site direct water consumption.}
Nearly all the server energy is converted into heat that must be removed
from the data center server room to avoid overheating. 
 Despite recent advances in cooling solutions,
cooling towers are dominantly the most common cooling solution
for warehouse-scale data centers, even for some leading companies such as
Google \cite{Google_Water} and  Microsoft \cite{Microsoft_Water_2023},
and consume a huge amount of water. 
As illustrated in Figure~\ref{fig:water_footprint},
there are two water loops: one closed loop between the chiller and 
data center server room, and one open loop between the cooling tower and the chiller.
Within the closed loop, water is not lost --- it is pumped from the chiller into the data center to cool down the air handling unit's supply
air in order to maintain a proper server inlet temperature, and
warm water that absorbs the server heat returns to the chiller direction.
Through a heat exchanger at the chiller, the heat is transferred from
the closed loop to the open loop. Note that the chiller may operate
in a ``bypass'' mode for energy saving when the outside temperature is low.
Along the open loop, some of the water gets evaporated (i.e., ``consumed'') in the cooling tower to dissipate heat into the environment. 
Additionally, there is a process called 
``blown down'' that drains the cooling water
to reduce salt concentration accumulated in the cooling tower and hence also consumes water:
the higher water quality, the more cycles of concentrations (i.e., water recirculates more times before ``blown down'') and hence the less blown-down water \cite{EDF_How_Cooling_Tower_Works}.
Through evaporation in the cooling tower  as well as ``blow down'', data centers consume a significant amount of freshwater. For example, by one estimate \cite{Water_WSJ_HiddenWaterUse_2015} and depending on climate conditions, 
roughly 3.8 liters of water are consumed
for each kWh of cooling load (approximately equal to server energy) by an
average data center, resulting in a water usage effectiveness (WUE) of 3.8 L/kWh,
while some data centers can even use 5.2 L/kWh \cite{Water_DataCenter_Beijing_Bank_2022}.
 Importantly, the on-site water comes from clean freshwater sources in order to avoid corrosion, clogged water pipes,
bacterial growth, etc.  
While air-side economizers (a.k.a. ``free'' outside air cooling)
do not need cooling towers and hence can reduce on-site water footprint,  they often have strict requirements on the climate condition and may
not be suitable for all locations. Additionally, freshwater is needed for humidity control to ensure proper server operation in data centers \cite{Facebook_WaterEfficiency_2012}.



\underline{Off-site indirect water consumption.}
Data centers are held accountable for carbon footprint because
of their (non-renewable) electricity usage. Likewise,
electricity generation requires a huge amount of water \cite{macknick2011review,Water_ElectricityGeneration_US_2003_torcellini2003consumptive},
thus resulting in off-site indirect water consumption for data centers
\cite{GreenGrid_Whitepaper_WUE}.
Depending on the cooling technologies employed, different power generation systems (e.g., nuclear, coal and natural gas) consume different amounts of water. Among the non-hydroelectric systems, nuclear power plants typically consume the highest amount of water for producing each kWh of electricity on average, followed by thermoelectricity \cite{macknick2011review}. The water efficiency metric
is called Energy Water Intensity Factor (EWIF) with a unit
of L/kWh.
 Although certain renewable energy generation such as wind turbine and solar PV panels consumes no water  for operation,  their percentages in the overall electricity generation is still low in most parts of the world.
Overall, excluding hydroelectricity (which itself does not consume water 
for cooling but expedites the evaporation of down streams),
the national average EWIF by aggregating different types of power plants in the U.S. is about 1.8 L/kWh \cite{GreenGrid_Whitepaper_WUE,Water_ElectricityGeneration_US_2003_torcellini2003consumptive}.








